Post-Quantum Security for Ultra-Reliable Low-Latency Heterogeneous Networks

We consider the problem of post-quantum secure and ultra-reliable communication through a heterogeneous network consisting of multiple connections. Three performance metrics are considered: security, throughput, and in-order delivery delay. In this setting, previous work has looked, individually, at the trade-offs between in-order delivery delay and throughput, and between security and throughput. This is the first work considering the trade-off between all three for heterogeneous communication networks, while taking the computational complexity into account. We present LL-HUNCC, a low latency hybrid universal network coding cryptosystem. LL-HUNCC is an efficient coding scheme which allows for secure communications over a noisy untrusted heterogeneous network by encrypting only a small part of the information being sent. This scheme provides post-quantum security with high throughput and low in-order delivery delay guarantees. We evaluate LL-HUNCC via simulations on a setting inspired by a practical scenario for heterogeneous communications involving a satellite communication link and a 5G communication network. Under this scenario, we compare LL-HUNCC to the state-of-the-art where all communication paths are encrypted via a post-quantum public-key cryptosystem.

==> tikz/secutiy_figure2.tex <==
\begin{tikzpicture}[scale=1]



% \draw [rounded corners] (0,0) rectangle (10,5);


\node[align=center] at (5,5) {\Large{Strong}};

\draw[-{Latex[length=2mm, width=2mm]}, color=black, thick] (5,4.6) -- (7.5,3.5);

\draw[-{Latex[length=2mm, width=2mm]}, color=black, thick] (5,4.6) -- (2.5,3.5);

\node[align=center] at (8,3) {\Large{Individual} ({\color{blue-violet}\textbf{I}})};

\node[align=center] at (2,3) {\Large{Post-Quantum} \\ \Large{Computational} ({\color{cerisepink}\textbf{C}})};

\draw[-{Latex[length=2mm, width=2mm]}, color=black, thick] (2.5,2.6) -- (4.5,1.5);

\draw[-{Latex[length=2mm, width=2mm]}, color=black, thick] (7.5,2.6) -- (5.5,1.5);

\node[align=center] at (5,1) {\Large{Post-Quantum} \\ \Large{Individual Computational} ({\color{cobalt}\textbf{IC}})};





\end{tikzpicture}
